Less Is More: Graph-free Multimodal RAG via Multi-signal Late Fusion

Graph-based retrieval-augmented generation (RAG) is widely used for multimodal, cross-document question answering. However, building corpus-level graphs is expensive, slow to query, and difficult to maintain. We present TrioRAG, a graph-free multimodal framework that integrates evidence from three complementary signals: the question, the anchor image, and a VLM-enhanced query generated from both. Each signal retrieves independently over a shared multi-vector index of page text and page images, and the results are combined through late fusion. Further, we introduce AutoQA, a multimodal automotive benchmark whose questions are grounded in noisy, web-sourced images rather than clean document-sourced figures. Its questions require reasoning across manuals. We position it as a model-curated testbed rather than a human-validated gold standard. Across three benchmarks, TrioRAG matches or outperforms graph-based systems while reducing total cost and accelerating per-query inference by 1.6-2.3 times. By construction, AutoQA grounds its questions in out-of-corpus web images. In this setting image retrieval reaches only 19.3% document-level recall, while text-derived signals, especially the VLM-enhanced query, keep retrieval robust.

==> tikz/motivation.tex <==

  % Old bitmap motivation figure (replaced by the TikZ version below):
% \includegraphics[width=\columnwidth]{images/motivation.png}
\begin{figure}[t]
  \centering
  \resizebox{\columnwidth}{!}{%
  \begin{tikzpicture}[
    font=\sffamily,
    >={Stealth[length=4pt]},
    cardbad/.style={draw=red!50!black, line width=0.6pt, rounded corners=3pt,
      fill=red!4, minimum width=41mm, minimum height=27mm},
    cardgood/.style={draw=teal!60!black, line width=0.6pt, rounded corners=3pt,
      fill=teal!5, minimum width=41mm, minimum height=27mm},
    ctitle/.style={font=\bfseries\small, anchor=north},
    cbody/.style={font=\footnotesize, align=left, anchor=north west, text width=25mm},
    pillbad/.style={draw=red!50!black, fill=red!8, rounded corners=4pt,
      font=\scriptsize, align=center, inner sep=2.5pt, text width=33mm, anchor=south},
    pillgood/.style={draw=teal!60!black, fill=teal!8, rounded corners=4pt,
      font=\scriptsize, align=center, inner sep=2.5pt, text width=33mm, anchor=south},
    seclbl/.style={font=\bfseries, anchor=west},
    % --- icons ---
    pics/clock/.style={code={
      \draw[red!60!black, line width=0.9pt] (0,0) circle (3.3mm);
      \draw[red!60!black, line width=0.9pt, line cap=round] (0,0) -- (0,2.1mm);
      \draw[red!60!black, line width=0.9pt, line cap=round] (0,0) -- (1.6mm,-0.2mm);
    }},
    pics/check/.style={code={
      \draw[teal!60!black, line width=1.5pt, line cap=round, line join=round]
        (-2.2mm,0.1mm) -- (-0.4mm,-1.9mm) -- (2.7mm,2.5mm);
    }},
    pics/quest/.style={code={
      \node[font=\bfseries\large, text=red!60!black] {?};
    }},
    pics/car/.style={code={
      \begin{scope}[teal!60!black]
        \fill[rounded corners=0.7mm] (-3.6mm,-0.7mm) rectangle (3.6mm,0.7mm);
        \fill (-2.0mm,0.5mm) -- (-1.1mm,1.8mm) -- (1.3mm,1.8mm) -- (2.1mm,0.5mm) -- cycle;
        \fill[white] (-2.1mm,-0.7mm) circle (1.0mm);
        \fill[white] (2.1mm,-0.7mm) circle (1.0mm);
        \fill (-2.1mm,-0.7mm) circle (0.5mm);
        \fill (2.1mm,-0.7mm) circle (0.5mm);
      \end{scope}
    }},
  ]

  %%%%%%%%%%%%%% Left: the worked example %%%%%%%%%%%%%%
  \node[align=center, font=\itshape, text width=33mm] (q) at (0,2.45)
    {``Why is my car leaking oil under the engine?''};
  \node[inner sep=0pt] (photo) at (0,0.05)
    {\includegraphics[width=33mm]{images/car_oil_leak.jpg}};
  \draw[rounded corners=2pt, line width=0.7pt, gray!55]
    (photo.south west) rectangle (photo.north east);
  % \node[font=\footnotesize\itshape, text=gray!55, anchor=north] at (photo.south)
  %   {a real, in-the-wild query};

  % dotted divider between example and comparison
  \draw[gray!50, line width=0.8pt, dash pattern=on 0.3pt off 1.7pt]
    (2.55,3.0) -- (2.55,-3.2);
  %%%%%%%%%%%%%% (a) speed comparison %%%%%%%%%%%%%%
  \node[seclbl] at (3.0,2.85) {(a)\, Graph pipelines are slow; ours stays simple and fast};
  % Graph-based card
  \node[cardbad] (ca) at (5.55,1.05) {};
  \node[ctitle, text=red!55!black] at ([yshift=-1.6mm]ca.north) {Graph-based RAG};
  \pic at ([xshift=-15.5mm,yshift=-12.5mm]ca.north) {clock};
  \node[cbody] at ([xshift=-11mm,yshift=-6.5mm]ca.north)
    {Complex pipeline $\Rightarrow$ high indexing \& inference time};
  \node[pillbad] at ([yshift=2.2mm]ca.south) {Graph creation is slow and brittle};
  % Ours card
  \node[cardgood] (cb) at (10.05,1.05) {};
  \node[ctitle, text=teal!60!black] at ([yshift=-1.6mm]cb.north) {Ours (graph-free)};
  \pic at ([xshift=-15.5mm,yshift=-12.5mm]cb.north) {check};
  \node[cbody] at ([xshift=-11mm,yshift=-6.5mm]cb.north)
    {Simple pipeline $\Rightarrow$ low indexing \& inference time};
  \node[pillgood] at ([yshift=2.2mm]cb.south) {No costly graph creation};

  %%%%%%%%%%%%%% (b) benchmark comparison %%%%%%%%%%%%%%
  \node[seclbl] at (3.0,-0.65) {(b)\, Existing benchmarks vs. AutoQA};
  % Existing benchmark card
  \node[cardbad] (cc) at (5.55,-2.45) {};
  \node[ctitle, text=red!55!black] at ([yshift=-1.6mm]cc.north) {Existing benchmarks};
  \pic at ([xshift=-15.5mm,yshift=-12.5mm]cc.north) {quest};
  \node[cbody] at ([xshift=-11mm,yshift=-6.5mm]cc.north)
    {Query images extracted from the source documents};
  \node[pillbad] at ([yshift=2.2mm]cc.south) {Queries do not reflect real-world conditions};
  % AutoQA card
  \node[cardgood] (cd) at (10.05,-2.45) {};
  \node[ctitle, text=teal!60!black] at ([yshift=-1.6mm]cd.north) {AutoQA (ours)};
  \pic at ([xshift=-15.5mm,yshift=-12.5mm]cd.north) {car};
  \node[cbody] at ([xshift=-11mm,yshift=-6.5mm]cd.north)
    {In-the-wild query images; cross-document QnA};
  \node[pillgood] at ([yshift=2.2mm]cd.south) {Real-world automotive troubleshooting};

  \end{tikzpicture}}
  \caption{The two problems we target, illustrated on a real query (left).
  (a) Graph-based multimodal RAG needs an expensive graph-construction pipeline
  (entity extraction, cross-modal alignment, graph building) and is slow and
  brittle, whereas our graph-free design embeds the corpus once and answers by
  retrieval and late fusion, cutting indexing and inference cost.
  (b) Existing benchmarks draw their query images from the source documents, so
  they do not reflect real-world conditions; AutoQA instead uses in-the-wild query
  images and cross-document questions drawn from real automotive troubleshooting.}
  \label{fig:motivation}
\end{figure}

==> tikz/motivation_data.tex <==
% Data-driven motivation figure (radar / spider chart).
% Three methods: Ours (graph-free), RAGAnything (graph-based), Naive RAG+Concat.
% Axes: three benchmark accuracies + three per-benchmark speeds, from Tables 1-2.
%
% Accuracy (multi-vector "M" rows of Table 1), axis scaled to 65%:
%   Ours        : MMLB 35.56  M3Sci 54.86  AutoQA 60.11
%   RAGAnything : MMLB 27.22  M3Sci 28.76  AutoQA 58.19
%   Naive RAG   : MMLB 35.56  M3Sci 20.69  AutoQA 45.31
% Speed = 1/(total time), normalized to the fastest run (Ours MMLB, 3.75 h):
%   Ours/Naive (graph-free, same index + single embedding pass): 3.75 / 5.93 / 5.31 h
%   RAGAnything (graph construction): 244.77 / 119.53 / 62.36 h
% Naive RAG is graph-free and shares our indexing+inference cost, so it
% coincides with Ours on the speed axes.
%
% To switch the paper to this version, change the \input in the Introduction
% from tikz/motivation.tex to tikz/motivation_data.tex.
\begin{figure}[t]
  \centering
  \resizebox{\columnwidth}{!}{%
  \begin{tikzpicture}[
    font=\sffamily,
    spoke/.style={gray!45, line width=0.4pt},
    grid/.style={gray!30, line width=0.3pt},
    axlbl/.style={font=\small, align=center, text=black},
    ours/.style={teal!60!black},
    graph/.style={red!65!black},
    naive/.style={orange!90!black},
    vtx/.style={circle, inner sep=0pt, minimum size=3pt},
  ]
    \def\R{2.4}

    % --- grid rings (hexagons at 25/50/75/100%) ---
    \foreach \lev in {0.25,0.5,0.75,1.0}{
      \draw[grid] (30:{\lev*\R}) \foreach \a in {90,150,210,270,330}{ -- (\a:{\lev*\R}) } -- cycle;
    }
    % --- spokes ---
    \foreach \a in {30,90,150,210,270,330}{ \draw[spoke] (0,0) -- (\a:\R); }
    \node[font=\footnotesize, text=gray!55, anchor=south west] at (90:\R) {\,100\%};

    % --- RAGAnything (graph) polygon ---
    \draw[graph, line width=1pt, fill=red!55, fill opacity=0.14]
      (30:2.149) -- (90:1.062) -- (150:1.005) -- (210:0.037) -- (270:0.075) -- (330:0.144) -- cycle;
    \foreach \a/\r in {30/2.149,90/1.062,150/1.005,210/0.037,270/0.075,330/0.144}{
      \node[vtx, fill=red!65!black] at (\a:\r){}; }

    % --- Ours polygon (filled, on top of graph) ---
    \draw[ours, line width=1.3pt, fill=teal!55, fill opacity=0.20]
      (30:2.220) -- (90:2.026) -- (150:1.313) -- (210:2.400) -- (270:1.518) -- (330:1.695) -- cycle;
    \foreach \a/\r in {30/2.220,90/2.026,150/1.313,210/2.400,270/1.518,330/1.695}{
      \node[vtx, fill=teal!60!black] at (\a:\r){}; }

    % --- Naive RAG polygon (dashed, no fill; coincides with Ours on speed) ---
    \draw[naive, line width=1.2pt, dash pattern=on 3pt off 2pt]
      (30:1.673) -- (90:0.764) -- (150:1.313) -- (210:2.400) -- (270:1.518) -- (330:1.695) -- cycle;
    \foreach \a/\r in {30/1.673,90/0.764,150/1.313}{
      \node[vtx, fill=orange!90!black] at (\a:\r){}; }

    % --- axis labels ---
    \node[axlbl, anchor=south]      at (90:{\R+0.34})  {M3SciQA\\{\footnotesize accuracy}};
    \node[axlbl, anchor=south east] at (150:{\R+0.30}) {MMLongBench\\{\footnotesize accuracy}};
    \node[axlbl, anchor=south west] at (30:{\R+0.30})  {AutoQA\\{\footnotesize accuracy}};
    \node[axlbl, anchor=north east] at (210:{\R+0.34}) {MMLongBench\\{\footnotesize speed}};
    \node[axlbl, anchor=north]      at (270:{\R+0.34}) {M3SciQA\\{\footnotesize speed}};
    \node[axlbl, anchor=north west] at (330:{\R+0.34}) {AutoQA\\{\footnotesize speed}};

    % --- speedup callouts on the speed axes (graph-free vs graph) ---
    \node[font=\small\bfseries, text=teal!50!black, anchor=east] at (210:{1.62}) {65$\times$};
    \node[font=\small\bfseries, text=teal!50!black, anchor=west] at (270:{1.08}) {20$\times$};
    \node[font=\small\bfseries, text=teal!50!black, anchor=west] at (330:{1.14}) {12$\times$};

    % --- legend (upper left) ---
    \begin{scope}[shift={(-5.0,3.85)}, font=\small]
      \draw[ours, line width=1.3pt, fill=teal!55, fill opacity=0.20] (0,0) rectangle (0.5,0.28);
      \node[anchor=west] at (0.62,0.14) {Ours};
      \draw[graph, line width=1pt, fill=red!55, fill opacity=0.14] (0,-0.5) rectangle (0.5,-0.22);
      \node[anchor=west] at (0.62,-0.86) {Naive RAG};
      \node[anchor=west] at (0.62,-0.36) {RAGAnything};
      \draw[naive, line width=1.2pt, dash pattern=on 3pt off 2pt] (0,-0.86) -- (0.5,-0.86);
      
    \end{scope}
  \end{tikzpicture}}
  \caption{Accuracy and per-benchmark speed for three methods
  (Tables~\ref{tab:main_results}, \ref{tab:efficiency}); each axis is normalized so
  larger is better. Our graph-free design covers the largest area, matching or
  exceeding both baselines on accuracy while being $12$--$65\times$ faster than the
  graph-based RAGAnything. Naive RAG shares our speed but trails on accuracy.}
  \label{fig:motivation}
\end{figure}

